The Area Method in the Wolfram Language

The area method is a decision procedure for geometry developed by Chou et al. in the 1990's. The method aims to reduce the specified hypothesis to an algebraically verifiable form by applying elimination lemmas. The order in which the lemmas are applied is determined by the stated conjecture and the underlying geometric construction. In this paper we present our implementation of the area method for Euclidean geometry as a stand-alone Mathematica package.

==> eptcsdata.tex <==
\providecommand{\firstpage}{64}
\providecommand{\publicationstatus}{Jani\v{c}i\'c, Kov\'acs (Eds.): Automated Deduction in Geometry (ADG 2021)\\
EPTCS 352, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.352.7}{10.4204/EPTCS.352.7}}
\pdfoutput=1

